Automated Testing of AI Models

The last decade has seen tremendous progress in AI technology and applications. With such widespread adoption, ensuring the reliability of the AI models is crucial. In past, we took the first step of creating a testing framework called AITEST for metamorphic properties such as fairness, robustness properties for tabular, time-series, and text classification models. In this paper, we extend the capability of the AITEST tool to include the testing techniques for Image and Speech-to-text models along with interpretability testing for tabular models. These novel extensions make AITEST a comprehensive framework for testing AI models.

==> back.tex <==
% !TEX root = main.tex
\section{Background}
\label{sec:back}


==> mymacros.tex <==
\usepackage{color}

\newtheorem{defn}{Definition}
\newcommand{\eat}[1]{} % comment
\newcommand{\remind}[1]{\textcolor{red}{\textsf{#1}}}


\newcommand{\BigCrunch}{\vspace{-1em}}
\newcommand{\Crunch}{\vspace{-0.8em}}
\newcommand{\SmallCrunch}{\vspace{-1ex}}
\newcommand{\Skip}{\vspace{1ex}}

\newcommand{\onefigure}[3]{
\begin{figure}[t]
\begin{center}
\centerline{\epsfxsize=0.98\columnwidth \epsffile{#1}}
\centerline{\parbox{\columnwidth}{\caption{#2} \label{#3}}}
\end{center}
\BigCrunch
\end{figure}
}

\newcommand{\onepdffigure}[3]{
    \begin{figure}[t] 
    \centerline{
    \includegraphics[scale=0.40]{#1}  
    }
    \vspace*{-1em}
    \centerline{
    \vspace*{-1.1em}
    \parbox{3.3in}{\caption{#2}
    \label{#3}}
    }
\end{figure}
}



\newcommand{\onelargepdffigure}[3]{
    \begin{figure}[t] 
    \centerline{
    \includegraphics[scale=0.37]{#1}  
    }
    \vspace*{-1em}
    \centerline{
    \vspace*{-1.1em}
    \parbox{3.3in}{\caption{#2}
    \label{#3}}
    }
\end{figure}
}

\newcommand{\onepdfigure}[3]{
    \begin{figure}[t] 
    \centerline{
    \includegraphics[scale=0.560]{#1}  
    }
    \vspace*{-1em}
    \centerline{
    \vspace*{-1.1em}
    \parbox{3.3in}{\caption{#2}
    \label{#3}}
    }
\end{figure}
}

\newcommand{\onesmallpdfigure}[3]{
    \begin{figure}[t] 
    \centerline{
    \includegraphics[scale=0.35]{#1}  
    }
    \vspace*{-1em}
    \centerline{
    \vspace*{-1.1em}
    \parbox{3.3in}{\caption{#2}
    \label{#3}}
    }
\end{figure}
}

\newcommand{\onemediumpdfigure}[3]{
    \begin{figure}[t] 
    \centerline{
    \includegraphics[scale=0.43]{#1}  
    }
    \vspace*{-1em}
    \centerline{
    \vspace*{-1.1em}
    \parbox{3.3in}{\caption{#2}
    \label{#3}}
    }
\end{figure}
}


\newcommand{\onetinyfigure}[3]{
\begin{figure}[t]
\begin{center}
\centerline{\epsfxsize=0.75\columnwidth \epsffile{#1}}
\centerline{\parbox{\columnwidth}{\vspace{-2em} \caption{#2} \label{#3}}}
\end{center}
\vspace{-4em}
\end{figure}
}

\newcommand{\onesmallfigure}[3]{
\begin{figure}[t]
\begin{center}
\centerline{\epsfxsize=0.85\columnwidth \epsffile{#1}}
\centerline{\parbox{\columnwidth}{\caption{#2} \label{#3}}}
\end{center}
\vspace{-2em}
\end{figure}
}


\newenvironment{my_enumerate}{
\begin{enumerate}
  \setlength{\itemsep}{1pt}
  \setlength{\parskip}{0pt}
  \setlength{\parsep}{0pt}}
{\end{enumerate}
}

\newenvironment{my_itemize}{
\begin{itemize}
  \setlength{\itemsep}{1pt}
  \setlength{\parskip}{0pt}
  \setlength{\parsep}{0pt}}
{\end{itemize}
}

\newcommand{\twofigs}[6]{
\begin{figure*}[t]
\centerline{
            \epsfxsize=3.0in \epsffile{#1}
            \hfill
            \epsfxsize=3.0in \epsffile{#4}
           }
\centerline{
            \parbox{3.0in}{\caption{#2} \label{#3}}
            \hfill
            \parbox{3.0in}{\caption{#5} \label{#6}}
           }
\Crunch
\end{figure*}
}

\newcommand{\twolargefigs}[6]{
\begin{figure*}[t]
\centerline{
            \includegraphics[scale=0.4]{#1}
     \hfill
    \includegraphics[scale=0.7]{#4}
           }
\centerline{
            \parbox{3.5in}{\caption{#2} \label{#3}}
            \hfill
            \parbox{3.5in}{\caption{#5} \label{#6}}
           }
\end{figure*}
}
{\newcommand{\twofigures}[6]{
\begin{figure*}[tbh]
\centerline{
            %\hfill
            \includegraphics[scale=0.49]{#1}
            \hfill
            \includegraphics[scale=0.49]{#2}
            %\hfill
           }
\vspace*{-1ex}
            \parbox{3in}{\centering (a)}
    \parbox{3in}{\centering (b)}
%%\Crunch
\vspace*{-1ex}
\centerline{
            %\hfill
            \parbox{9.0in}{\caption{#3} \label{#4}}
            \hfill
          %%  \parbox{3.0in}{\caption{#5} \label{#6}}
          %%  %\hfill
           }
\Crunch
\end{figure*}
% \Skip
}


{\newcommand{\twolargefigures}[6]{
\begin{figure*}[tbh]
\centerline{
            %\hfill
            \includegraphics[scale=0.41]{#1}
            \hfill
            \includegraphics[scale=0.51]{#2}
            %\hfill
           }
\vspace*{-1ex}
            \parbox{3in}{\centering (a)}
    \parbox{3in}{\centering (b)}
%%\Crunch
\vspace*{-1ex}
\centerline{
            %\hfill
            \parbox{9.0in}{\caption{#3} \label{#4}}
            \hfill
          %%  \parbox{3.0in}{\caption{#5} \label{#6}}
          %%  %\hfill
           }
\Crunch
\end{figure*}
% \Skip
}


\newcommand{\twoabsinglecolumnfigures}[5]{
    \begin{figure}[!tbh]
    \centerline{
    \includegraphics[scale=0.2]{#1}
    \hfill
    \includegraphics[scale=0.2]{#2}
    }
    \parbox{0.45\columnwidth}{\centering (a) 10 node cluster}
    \parbox{0.45\columnwidth}{\centering (b) 30 node cluster}
    \centerline{
    \parbox{9in}{\caption{#3}
    \label{#4}}
    \hfill
    }
\vspace{-0.2in}
%\Crunch
%    \DoubleSpace
%\Skip
\end{figure}
}



\newcommand{\threefiguressmaller}[5]{
    \begin{figure*}[tbh]
    \centerline{
    \includegraphics[scale=0.37]{#1}
    \hfill
    \includegraphics[scale=0.37]{#2}
    \hfill
    \includegraphics[scale=0.37]{#3}
    }
\vspace{-0.6em}
%    \SingleSpace
     \parbox{2.31in}{\centering (a)}
    \parbox{2.46in}{\centering (b)}
    \parbox{2.4in}{\centering (c)}    \centerline{
    \parbox{9in}{\caption{#4}
    \label{#5}}
    \hfill
    %%\parbox{2.15in}{\caption{#5}
   %% \label{#6}}
   %% \hfill
    %%\parbox{2.15in}{\caption{#8}
   %% \label{#9}}
    }
\vspace{-0.2in}
%\Crunch
%    \DoubleSpace
%\Skip
\end{figure*}
}




\eat{\newcommand{\threefigures}[9]{
    \begin{figure*}[tbh]
    \centerline{
    \epsfxsize=2.4in \epsffile{#1}
    \hfill
    \epsfxsize=2.4in \epsffile{#4}
    \hfill
    \epsfxsize=2.4in
    \epsffile{#7}
    }
\vspace{-1em}
%    \SingleSpace
    \centerline{
    \parbox{2.15in}{\caption{#2}
    \label{#3}}
    \hfill
    \parbox{2.15in}{\caption{#5}
    \label{#6}}
    \hfill
    \parbox{2.15in}{\caption{#8}
    \label{#9}}
    }
\Crunch
%    \DoubleSpace
\Skip
\end{figure*}
}}

\newcommand{\fourfigures}[8]{
    \begin{figure*}[thb]
    \centerline{
    \epsfxsize=1.575in \epsffile{#1}
    \hfill
    \epsfxsize=1.575in \epsffile{#2}
    \hfill
    \epsfxsize=1.575in \epsffile{#5}
    \hfill
    \epsfxsize=1.575in \epsffile{#6}
    }
%    \SingleSpace
\SmallCrunch
    \centerline{
    \parbox{3.2in}{\caption{#3} \label{#4}}
    \hfill
    \parbox{3.2in}{\caption{#7} \label{#8}}
    }

%    \DoubleSpace
\Skip
\end{figure*}
}

\newenvironment{my_description}{
\begin{description}
  \setlength{\itemsep}{1pt}
  \setlength{\parskip}{0pt}
  \setlength{\parsep}{0pt}}
{\end{description}}

\newenvironment{mylist}{
% \baselineskip 10 pt
\begin{list}{$\bullet$}{
\setlength{\leftmargin}{1.5ex}
\setlength{\labelwidth}{1ex}
\setlength{\labelsep}{0.5ex}
\setlength{\itemsep}{0.2ex}
\setlength{\parsep}{0.2ex}
}}
{\end{list}}


==> property_tds.tex <==

\begin{algorithm}[htb]
\scriptsize
\SetAlgoLined
\SetAlgoLined\DontPrintSemicolon

    \SetKwFunction{FMain}{synthesize}
  \SetKwProg{Fn}{function}{:}{}
  \Fn{\FMain{train\_data, n, class\_label, property, protected\_attr=None}}{ \label{func:synthesize}
        constraints = get\_constraints(train\_data) \\
        feature\_order = get\_process\_order(constraints, class\_label, property, protected\_attr)\\
       //same as lines ~\ref{line:st}-~\ref{line:ed} in Algorithm ~\ref{algo:generate} \\
        \KwRet synth\_data
    }
  
    \SetKwFunction{FMain}{get\_process\_order}
    \SetKwProg{Fn}{function}{:}{}
    \Fn{\FMain{constraints, class\_label, property, protected\_attr=None}}{ \label{func:gpo_prop}
        constraints.remove\_feature(class\_label)\\ \label{line:label}
        \uIf{property $\in$ \{GROUP\_FAIRNESS\}}{ \label{line:fair}
            constraints.remove\_associations(protected\_attr)
        }
        g = create\_graph(constraints.feature\_names)\\
        g.add\_all\_edges(constraints.associations)\\
        g = preprocess(g)\\
        feature\_order = topological\_sort(g)\\
        \KwRet feature\_order
    }

\caption{Property based Test Input Generation}\label{algo:fairness}
  
\end{algorithm}

As mentioned in Section~\ref{sec:arch}, we further intend to generate realistic test cases to test an input AI model for a number of properties, namely, \emph{Correctness}, \emph{Individual Fairness}, \emph{Group Fairness} and \emph{Robustness}. We use the same base approach as presented above with a few changes depending on the property. The required algorithmic changes are concerned only with the user inputs, and the implementation of method \texttt{gen\_process\_order}, as presented in Algorithm ~\ref{algo:fairness}. Following are the user inputs required for property-based test inputs generation to test an AI model.
\begin{itemize}
    \item \textit{data} - training data from which data constraints are fetched.
    \item \textit{n} - count of required test inputs to be generated.
    \item \textit{class\_label} - feature name in the input data containing the decision class values.
    \item \textit{property} - AI model test property for which test inputs need to be generated.
    \item \textit{protected\_attr} - name of the protected or sensitive attributes such as gender, race, etc. present in the input training data, based on which the input AI model is not supposed to take any decision in an ideal scenario. Please note that this is a mandatory user input only for Individual and Group Fairness property use cases. 
\end{itemize}
For the property based test input generation given in Algorithm ~\ref{algo:fairness}, the method \texttt{gen\_process\_order} starts with removing the feature related to input class label along with all the association constraints where this feature is specified as either a source or target (line ~\ref{line:label}). This is done to make sure that any approximation caused due to constraint inference or synthesis does not seep into the prediction labels for these test inputs.

\subsubsection{Correctness Test Case Generator}
Since we generate test inputs conforming to the behaviour/constraints inherent in the input training data, therefore, these realistic test inputs, of reasonably good size, should be able to cover most of the paths of the trained model. Hence, they can be put to test correctness of an input AI model too. As mentioned earlier, we don't use constraints to synthesize prediction values for these realistic test cases. Label assignment ideally should be a done by manual intervention, but, we instead use a \emph{Multi-model Label Generator} to guess labels for these inputs.
\input{label_generator}


\subsubsection{Individual Fairness Test Case Generator}
As mentioned earlier in Section~\ref{sec:back}, we employ an existing approach \cite{testing-fse} to generate test cases for individual fairness testing of a black-box AI model. The process of generation involves the following two phases.\\
\textit{Global Search} - First, we synthesize required number of test cases by satisfying data constraints, which constitute the set of global inputs. \\ 
\textit{Local Search} - The global inputs are then clustered and processed one by one according to the strategy in \cite{testing-fse}. Once a discriminatory test case, say t, is found, we try to generate further more test inputs in its neighborhood which may lead to uncover individual discrimination. 
We use an off-the-shelf explainer LIME~\cite{LIME} to get a set of top $50\%$ attributes contributing to the explanation of test case, t. For every prominent attribute, say a, we then generate further more local test inputs by perturbing its value as per the below scheme based on its datatype.\\
\emph{CAT\_TEXT/CAT\_NUM}: Generate inputs by perturbing t[a] for all possible values. \\
\emph{NUMERIC/FLOAT}: Generate inputs by perturbing t[a] for all integers or floats in range (t[a]-3, t[a]+3). Please note that the perturbation in such cases are bounded by the minimum and maximum permissible bounds of attribute a inferred from data constraints.
\subsubsection{Group Fairness Test Case Generator} 
Specifically just for the group fairness use case, in addition to class label, we further unconditionally make the protected feature independent by removing all those associations from the data constraints where it is mentioned as the target (line ~\ref{line:fair}). This is done to ensure that the protected attribute in resultant synthetic test inputs follow the same frequency distribution as that of the input training data set. For example, if the training data has composition of males and females in the ratio 2:1, then, it is desirable to test the model for group fairness with the test cases having same 2:1 male female ratio. Please note that this frequency distribution of protected attribute can be over-ridden by means of user-specified constraints as well as mentioned earlier in Subsection~\ref{sec:user-defined}.
\subsubsection{Robustness Test Case Generator}
Except for the class label, we synthesize realistic data satisfying all the feature and association constraints. For every realistic test, say t, we then perform robustness testing of the input model by generating more inputs in its neighbourhood, and checking if the predictions of any neighbour is different than t's. Please note that we use the same definition of neighborhood as the one used in Individual Fairness Test Generator.

==> proptable.tex <==
\begin{table}[t]
  \caption{Test Properties for different Model Types}
\centering
 \begin{tabular}{|l|l|p{0.25\linewidth}|}\hline`
Test Property & Metrics & Test Failure\\\hline
\multicolumn{3}{|c|}{Tabular data Classifier}\\\hline
Correctness & Accuracy & \multirow{4}{=}{Label mismatch with gold standard label}\\
  & Precision & \\
  & Recall & \\
  & F-Score & \\\hline
Group Discrimination (R) & Disparate Impact (DI) & \multirow{2}{=}{If DI $\notin R$}\\
  & Demographic Parity & \\\hline
Individual Discrimination & \multirow{2}{*}{Flip-rate} & \multirow{2}{=}{Label mismatch of the two samples}\\\cline{1-1}
Adversarial Robustness &  & \\\hline
\multicolumn{3}{|c|}{Text Classifier}\\\hline
Typo Sensitivity(L) & \multirow{6}{*}{Flip-rate} & \multirow{6}{=}{Label mismatch of original and transformed sample} \\\cline{1-1}
Noise Sensitivity(L) & & \\\cline{1-1}
Adjective Sensitivity & & \\\cline{1-1}
Tense Sensitivity & & \\\cline{1-1}
Voice Sensitivity & & \\\cline{1-1}
Paraphrase variation & & \\\hline
\multicolumn{3}{|c|}{Time Series Forecasting}\\\hline
Small Linear Change ($\alpha$) &  \multirow{3}{*}{RMSE change ($\Delta R$)} & \multirow{2}{=}{If $\Delta R > \alpha$}\\\cline{1-1}
Un-ordered data ($\alpha$) & &\\\cline{1-1}\cline{3-3}
Large Linear Change ($\beta$) &  & If $\Delta R < \beta$ \\\hline
  \end{tabular}
  \label{tab:1}
\end{table}

\eat{
\begin{table*}[t]
  \centering
  \begin{tabular}{|p{0.10\linewidth}|p{0.20\linewidth}|p{0.20\linewidth}|p{0.20\linewidth}|p{0.20\linewidth}|}
    \hline
Modality & Test Property & Metric & Failure case & Action \\
\hline
\hline
Text & Robustness of model to various perturbations to input text. Perturbations include:
\begin{itemize}[leftmargin=*]
\item Addition of typos
\item Addition of noise
\item Variations in tense, voice, adjective intensity
\item Adversarial variations using back-translation
\end{itemize}
&
Flip rate of the class label
&
Class label should not change for perturbations –the label before and after perturbation should be the same.
&
Based on \%age of flips of class labels, retraining with additional data is recommended.\\
\hline
Conversation &
Static analysis to check for possible errors  in the chatbot attributes –entities,  intents and dialog nodes. &
Fractions of:
\begin{itemize}[leftmargin=*]
\item Intents with less examples
\item Intents with no verbs
\item Short intents
\item Intents with invalid relations
\item Dialog nodes that can pre-emptively end a conversation
\end{itemize} &

If any fraction is above a user-defined threshold, that test case is a failure. &
Report the findings for relevant action.
\\
\hline
\multirow{4}{\linewidth}{Tabular data} & Individual Fairness & Flip rate of the class label (with change in protected attribute values) & For any sample input, class label should not change with change in value of protected attribute – the label before and after perturbation should be the same. & \\ \cline{2-5}

&Group Fairness & 
\begin{itemize}[leftmargin=*]
\item Disparate impact
\item Demographic parity
\end{itemize} & If the value of disparate impact is less than the user-defined threshold (say 0.8), it is a failure & \\ \cline{2-5}
& Robustness & Flip rate of the class label (for synthetic neighboring samples) & For any sample, the class label should not change for neighboring perturbations – the label before and after perturbation should be the same. & \\ \cline{2-5} 
& Prediction Accuracy & Accuracy Score & For any sample, if its model prediction differs from the ground truth, then it's a failure & \\ \hline
\multirow{4}{\linewidth}{Time series} & Small (adversarial) linear change & RMSE gain & If RMSE gain is more than 10\%, it's a failure & Retrain with more regularization \\ \cline{2-5}
& Large Linear Change (Adding 10*(max-min) to each instance) & If RMSE gain is less than less than 10\%, it's a failure & Do not normalize with the min-max of the test data. \\ \cline{2-5}
& Zero-ranged data & Status code of API call & If the API call fails with any status code apart from 200, it's a failure & Do not normalize with the min-max of the test data. \\ \cline{2-5}
& Un-ordered data & RMSE gain & If RMSE gain is greater than 0, it's a failure & Sort the data with timestamp before attempting to forecast.\\
\hline
  \end{tabular}
  \caption{Various test properties and corresponding metrics associated with all the supported modalities}
  \label{tab:1}
\end{table*}
}

==> synthesis_algo.tex <==
\begin{algorithm}[htb]
\scriptsize
\SetAlgoLined
\SetAlgoLined\DontPrintSemicolon

\SetKwFunction{FMain}{synthesize}
  \SetKwProg{Fn}{function}{:}{}
  \Fn{\FMain{constraints, n}}{ \label{func:synthesize}
        % constraints = get\_constraints(data) \\
        feature\_order = get\_process\_order(constraints)\\ \label{line:process}
        synth\_data = \{ \}\\ \label{line:st}
        \ForEach {feature $f$ in feature\_order}{
            \uIf{is\_independent(f, constraints)}{
                synth\_vals = gen\_by\_feature\_constraints(f, n)
            }
            \uElse{
            assocs = constraints.get\_all\_associations(f) \\ \label{line:assoc}
 synth\_vals = gen\_by\_associations(f, assocs, synth\_data, n)
            }
            synth\_data[f] = synth\_vals 
        } \label{line:ed}
        \KwRet synth\_data
    }
  
    \SetKwFunction{FMain}{get\_process\_order}
    \SetKwProg{Fn}{function}{:}{}
    \Fn{\FMain{constraints}}{ \label{func:get_order}
        g = create\_graph(constraints.feature\_names)\\
        g.add\_all\_edges(constraints.associations)\\
        g = preprocess(g)\\
        feature\_order = topological\_sort(g)\\
        \KwRet feature\_order
    }
    
    \SetKwFunction{FMain}{is\_independent}
    \SetKwProg{Fn}{function}{:}{}
    \Fn{\FMain{feature, constraints}}{ \label{func:get_order}
        assocs = constraints.get\_all\_associations(feature)\\
        \uIf{ assocs is None}{
            \KwRet True
        }
        \KwRet False
    }


    \SetKwFunction{FMain}{gen\_by\_feature\_constraints}
    \SetKwProg{Fn}{function}{:}{}
    \Fn{\FMain{feature $f$, n}}{ \label{func:gen_by_features}
        \uIf{f.datatype $\in$ \{NUMERIC, FLOAT\}}{
            dist = f.distribution\\
            \uIf{dist is None}{
                vals = draw\_samples(UNIFORM, f.min, f.max, f.is\_unique, n)
            }
            \uElse{
            vals = draw\_samples(dist.name, dist.parameters, f.min, f.max, f.is\_unique, n)
            }
        }
        \uElseIf{feature.datatype $\in$ \{CAT\_TEXT or CAT\_NUM\}}{
            \uIf{feature.frequency is None}{
            vals = gen\_randomly(f.possible\_vals, n)
            }
            \uElse{
            vals = gen\_by\_freqDist(f.frequency, n)
            }
        }
        \uElseIf{feature.datatype is TEXT}{
            vals = gen\_by\_regex(f.pattern, f.min\_len, f.max\_len, f.is\_unique, n)
        }
        \uElseIf{feature.datatype is DATE}{
            vals = gen\_dates\_between(f.start\_date, f.end\_date, f.format, 
            f.is\_unique, n)
        }
        \KwRet vals
    }

\SetKwFunction{FMain}{gen\_by\_associations}
\SetKwProg{Fn}{function}{:}{}
\Fn{\FMain{feature $f$, assocs, synth\_data, n}}{ \label{func:gen_by_assocs}
    \uIf{feature.datatype $\in$ \{NUMERIC, FLOAT\}}{
        numnum\_assocs = assocs.get\_by\_type(NUM-NUM)\\
        catnum\_assocs = assocs.get\_by\_type(CAT-NUM)\\
        \uIf{numnum\_assocs is not None}{
            vals = gen\_by\_numnum(f, numnum\_assocs, assocs, synth\_data, n)\\
         }
        
        \uElseIf{catnum\_assocs is not None}{
            vals = gen\_by\_catnnum(f, catnum\_assocs, synth\_data, n)\\
        }
        
    }
    \uIf{feature.datatype $\in$ \{CAT\_TEXT, CAT\_NUM\}}{
        vals = gen\_by\_catcat(f, assocs, synth\_data, n)\\
    }
    
    \uIf{feature.datatype is DATE}{
        vals = gen\_by\_datedate(f, assocs, synth\_data, n)\\
    }
    \KwRet vals
}

\caption{Realistic Data Synthesis}\label{algo:generate}
  
\end{algorithm}




\begin{algorithm}[htb]
\scriptsize
\SetAlgoLined
\SetAlgoLined\DontPrintSemicolon

\SetKwFunction{FMain}{gen\_by\_numnum}
\SetKwProg{Fn}{function}{:}{}
\Fn{\FMain{feature $f$, numnum\_assocs, catnum\_assocs, synth\_data, n}}{ \label{func:gen_by_numnum}
    solver = Solver()\\
    \ForEach{assoc $\in$ numnum\_assocs}{
             equations = form\_equations(assoc, synth\_data[assoc.source])\\
             solver.add(equations)\\
    }
     vals = solver.solve(f.is\_unique)\\
     
     isValid, invalid\_idxs = validate(val, catnum\_assocs, feature)\\
        \uIf{!isValid}{
            \ForEach{idx $\in$ invalid\_idxs}{
                vals[idx] = gen\_by\_catnum($f$, catnum\_assocs, synth\_data, n=1)
            }
        }
     \KwRet vals
}

\SetKwFunction{FMain}{gen\_by\_catnum}
\SetKwProg{Fn}{function}{:}{}
\Fn{\FMain{feature $f$, catnum\_assocs, synth\_data, n}}{ \label{func:gen_by_catnum}
        vals = []\\
        \ForEach{srcval $\in$ synth\_data[assoc.source]}{
            assoc = pick\_max\_overlap\_catnum(catnum\_assocs, srcval) \\
            dist = assoc.get\_dist\_by\_src(srcval)\\ trials=0, success=False\\
            \While{!success and trials < MAX\_TRIALS}{
                val = draw\_samples(dist.name, dist.parameters,f.min,f.max, n=1)\\
                \uIf{f.is\_unique and is\_exists(val, vals)}{
                    trails++, continue
                }
                isValid = validate(val, catnum\_assocs, feature)\\
                \uIf{isValid}{success=True}
                trail++
            }
            \uIf{!success}{
                val = gen\_by\_feature\_constraints(feature=f, n=1)
            }
            vals.append(val)
        }
}


\SetKwFunction{FMain}{gen\_by\_catcat}
\SetKwProg{Fn}{function}{:}{}
\Fn{\FMain{feature $f$, assocs, synth\_data, n}}{ \label{func:gen_by_catcat}
    assoc = pick\_any\_randomly(assocs) \\
    src\_vals = synth\_data[assoc.source]\\
    vals = gen\_by\_freq(assoc.frequency, src\_vals) \\
    \KwRet vals
}



\SetKwFunction{FMain}{gen\_by\_datedate}
\SetKwProg{Fn}{function}{:}{}
\Fn{\FMain{feature $f$, assocs, synth\_data, n}}{ \label{func:gen_by_datedate}
    \ForEach{assoc $\in$ assocs}{
        src\_vals = synth\_data[assoc.source]\\
        solver = datesolver(), i=0\\
        \While{i $<$ n}{
            solver.add($val_{i}$ $==$ $src\_val_{i}$ $+$ $delta_{i}$)\\
            solver.add($delta_{i}$ $>=$ $assoc.min\_diff$)\\
            solver.add($delta_{i}$ $<=$ $assoc.max\_diff$)\\
            solver.add($val_{i}$ $>=$ $f.start\_date$)\\
            solver.add($val_{i}$ $<=$ $f.end\_date$), i++\\
         }
        } 
    
    vals = solver.solve(unique=f.is\_unique), i=0 \\
    //fallback\\
    \While{i $<$ n}{     
        \uIf{$vals[i]$ is None}{
            vals[i] = gen\_by\_feature\_constraints(f, n=1)
        }
    }
    \KwRet vals
    }
}


\caption{Synthesis Using Associations} \label{algo:synth_assocs}
\end{algorithm}

==> ui.tex <==
\section{User Interaction and Tooling}
\label{sec:ui}

%\begin{figure}[t]
%\centering
%\includegraphics[height=4.5cm, width=9cm]{images/register.png}
%\caption{Model Registration}
%\label{fig:register}
%\end{figure}

%\begin{figure}[t]
%\centering
%\includegraphics[ width=9cm]{images/config.png}
%\caption{Test Configuration}
%\label{fig:config}
%\end{figure}

%\begin{figure}[t]
%\centering
%\includegraphics[ width=9cm]{images/runs.png}
%\caption{Test Runs}
%\label{fig:runs}
%\end{figure}

%\begin{figure}[t]
%\centering
%\includegraphics[ width=9cm]{images/metrics.png}
%\caption{Test Metrics}
%\label{fig:metric}
%\end{figure}

% \begin{figure}[t]
% \centering
% \includegraphics[height=4.5cm, width=9cm]{images/failures.png}
% \caption{Test Failures}
% \label{fig:fail}
% \end{figure}

% \begin{figure}[t]
% \centering
% \includegraphics[height=4.5cm, width=9cm]{images/compare.png}
% \caption{Run Comparison}
% \label{fig:compare}
% \end{figure}


In this section, we present a demo scenario for tabular modality by considering an input model from Bank Marketing domain. Such an input model defined by means of an API, and hence black-box in nature is first registered by the user with the tester, as shown in Fig.~\ref{fig:register}. The model once registered, can then be tested by creating a new run configuration or re-running an existing one, refer Fig.~\ref{fig:config}. The user needs to enter certain data specific parameters, such as protected attribute, favorable prediction and minority group required for fairness-related property testing along with an optional user-defined constraints. This test run is then saved and executed after selecting the desired properties to be tested and specifying the test generation limit. The status of this run is dynamically updated on the Manage Test Runs tab in Fig.~\ref{fig:runs}, where different statistics regarding how many test cases have been generated, executed, passed or failed a particular property testing are recorded and refreshed. For every tested property, the user can access the overall test evaluation on the basis of different metric calculation along with an associated explanation and heat-map visualization summary for better understanding, see Fig.~\ref{fig:metric}.
The interface further allows the user to drill down these results and view the test cases which have failed the selected property testing. Fig.~\ref{fig:fail} shows such test cases marked as \textit{original} which have failed Individual Discrimination Testing. The  tests with header \textit{transformed} are the perturbations of that of \textit{original}, which differ only in the protected attribute i.e. \textit{marital}, but yield different predictions. The tool also exposes a comparative view (Fig.~\ref{fig:compare}) which enables the user to compare the results of different test runs having different test configurations and help him/her choose the best performing one at finding bugs.

The framework has been tested in various modalities as under:
\begin{enumerate}
    \item Conversation: It has been tested on $6$ production-level conversation scenarios.
    \item Text: It has been integrated with a business platform for improving AI productivity.
    \item Time series: It has been tested on simple ARIMA \cite{weiss2000forecasting} and LSTM \cite{hochreiter1997long} models trained on open-source datasets \cite{van1999cluster} \cite{keogh2005hot} \footnote{The ECG dataset from \cite{keogh2005hot} can be found here: http://www.cs.ucr.edu/~eamonn/discords/}.
    \item Tabular: The work specific to tabular data has been submitted as a full-length paper in the Industrial track of this conference~\cite{our paper}
\end{enumerate}
